On the Impact of Operators and Populations within Evolutionary Algorithms for the Dynamic Weighted Traveling Salesperson Problem

Evolutionary algorithms have been shown to obtain good solutions for complex optimization problems in static and dynamic environments. It is important to understand the behaviour of evolutionary algorithms for complex optimization problems that also involve dynamic and/or stochastic components in a systematic way in order to further increase their applicability to real-world problems. We investigate the node weighted traveling salesperson problem (W-TSP), which provides an abstraction of a wide range of weighted TSP problems, in dynamic settings. In the dynamic setting of the problem, items that have to be collected as part of a TSP tour change over time. We first present a dynamic setup for the dynamic W-TSP parameterized by different types of changes that are applied to the set of items to be collected when traversing the tour. Our first experimental investigations study the impact of such changes on resulting optimized tours in order to provide structural insights of optimization solutions. Afterwards, we investigate simple mutation-based evolutionary algorithms and study the impact of the mutation operators and the use of populations with dealing with the dynamic changes to the node weights of the problem.

==> tables/compressed_results.tex <==
\begin{table*}[htbp]
\caption{\label{tab:all_results}Mean (\textbf{mean}), standard deviation (\textbf{std}) and results of Wilcoxon-Mann-Whitney tests at a significance level of $\alpha = 0.05$ (\textbf{stat}) in terms of relative performance for all considered instances. Best, i.e. lowest, mean values are highlighted in \colorbox{gray!20}{\textbf{bold face}}. The entries in the stat-column are read as follows: a value of $S \in \{1, \ldots, 6\}$ means that algorithm $S$ performs significantly worse. Interval notation $S-T$ means that all algorithms in the interval perform worse.}
\renewcommand{\arraystretch}{0.85}
\renewcommand{\tabcolsep}{5.7pt}
\centering
\begin{scriptsize}
%\begin{tiny}
\begin{tabular}[t]{crrrrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{9}{c}{\textbf{(1+1) EA}} & \multicolumn{9}{c}{\textbf{(20+1)-EA}} \\
\cmidrule(l{3pt}r{3pt}){5-13} \cmidrule(l{3pt}r{3pt}){14-22}
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{3}{c}{\textbf{Inversion (1)}} & \multicolumn{3}{c}{\textbf{Swap (2)}} & \multicolumn{3}{c}{\textbf{Jump (3)}} & \multicolumn{3}{c}{\textbf{Inversion (4)}} & \multicolumn{3}{c}{\textbf{Swap (5)}} & \multicolumn{3}{c}{\textbf{Jump (6)}} \\
\cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10} \cmidrule(l{3pt}r{3pt}){11-13} \cmidrule(l{3pt}r{3pt}){14-16} \cmidrule(l{3pt}r{3pt}){17-19} \cmidrule(l{3pt}r{3pt}){20-22}
& $\tau$ & $[L, U]$ & $c$ & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat}\\
\midrule
 &  &  & 2 & 22.8 & 9.5 & 3-6 & \cellcolor{gray!20}{\textbf{16.0}} & 7.3 & 1,3-6 & 38.0 & 11.2 &  & 39.7 & 30.0 &  & 40.0 & 19.2 &  & 35.7 & 17.7 & 4-5\\

 &  &  & 5 & 18.8 & 9.0 & 3-6 & \cellcolor{gray!20}{\textbf{15.6}} & 7.6 & 3-6 & 43.8 & 14.3 &  & 41.6 & 29.6 & 5 & 44.9 & 18.7 &  & 38.6 & 18.3 & 3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 16.7 & 10.0 & 3-6 & \cellcolor{gray!20}{\textbf{15.3}} & 8.1 & 3-6 & 49.2 & 16.7 &  & 45.8 & 30.5 & 3,5 & 50.2 & 19.2 &  & 42.6 & 19.0 & 3-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{19.1}} & 6.7 & 3-6 & 21.8 & 6.1 & 3-6 & 35.3 & 7.8 &  & 34.3 & 30.4 & 5 & 40.2 & 20.0 &  & 30.0 & 19.4 & 3-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{13.3}} & 5.6 & 2-6 & 19.2 & 6.6 & 3-6 & 31.5 & 8.4 & 5 & 34.1 & 29.7 & 5 & 41.1 & 20.4 &  & 29.1 & 19.4 & 3-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$10\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{11.5}} & 6.1 & 2-6 & 19.2 & 7.3 & 3-6 & 29.5 & 10.1 & 5 & 33.7 & 30.1 & 5 & 42.0 & 21.1 &  & 32.7 & 19.5 & 5\\

\cmidrule{2-22}
 &  &  & 2 & 20.8 & 8.1 & 3 & 15.6 & 7.1 & 3 & 38.2 & 11.4 &  & 3.0 & 10.8 & 1-3,5 & 11.0 & 9.3 & 2-3 & \cellcolor{gray!20}{\textbf{-0.3}} & 12.4 & 1-5\\

 &  &  & 5 & 15.9 & 8.7 & 3 & 14.0 & 7.5 & 3 & 38.8 & 13.1 &  & 3.6 & 11.1 & 1-3,5 & 12.3 & 9.6 & 3 & \cellcolor{gray!20}{\textbf{1.5}} & 10.7 & 1-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 15.4 & 9.9 & 3 & 9.3 & 7.3 & 3,5 & 42.7 & 16.4 &  & \cellcolor{gray!20}{\textbf{4.6}} & 11.3 & 1-3,5 & 12.7 & 9.9 & 3 & 5.5 & 10.2 & 1-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 14.2 & 5.8 & 2-3 & 21.1 & 5.9 & 3 & 33.4 & 7.3 &  & 1.7 & 10.6 & 1-3,5 & 13.9 & 9.4 & 2-3 & \cellcolor{gray!20}{\textbf{-0.9}} & 11.9 & 1-5\\

 &  &  & 5 & 13.8 & 6.3 & 3 & 14.4 & 6.4 & 3 & 29.3 & 7.7 &  & 0.6 & 10.4 & 1-3,5 & 12.9 & 9.4 & 3 & \cellcolor{gray!20}{\textbf{-0.6}} & 11.4 & 1-5\\

\multirow{-14}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{eil101-bsc}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$75\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 13.2 & 6.0 & 3 & 16.2 & 6.2 & 3 & 28.4 & 8.5 &  & 0.8 & 10.9 & 1-3,5 & 12.4 & 9.9 & 2-3 & \cellcolor{gray!20}{\textbf{0.2}} & 11.6 & 1-3,5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{15.4}} & 7.0 & 2-6 & 21.5 & 7.0 & 3-6 & 41.2 & 10.7 &  & 38.1 & 29.3 & 5 & 41.7 & 19.0 &  & 32.5 & 18.4 & 3-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{16.8}} & 8.7 & 3-6 & 17.9 & 8.1 & 3-6 & 42.8 & 12.1 &  & 39.6 & 29.4 & 3,5 & 46.3 & 19.4 &  & 36.7 & 18.2 & 3-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{15.1}} & 7.3 & 3-6 & 16.0 & 7.7 & 3-6 & 45.2 & 15.4 &  & 43.8 & 28.7 & 5 & 50.9 & 18.5 &  & 40.4 & 18.3 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{14.8}} & 4.9 & 3-6 & 19.6 & 5.6 & 3-6 & 32.6 & 6.7 & 5 & 32.3 & 29.6 & 5 & 42.6 & 20.9 &  & 29.9 & 18.9 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{11.7}} & 5.7 & 2-6 & 21.9 & 6.5 & 3-6 & 27.3 & 7.9 & 4-6 & 32.3 & 29.0 & 5 & 44.3 & 21.6 &  & 30.3 & 19.1 & 4-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$10\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{8.4}} & 6.8 & 2-6 & 18.7 & 7.3 & 3-6 & 29.7 & 8.4 & 5 & 33.4 & 29.9 & 5 & 43.9 & 21.4 &  & 31.4 & 18.7 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & 17.8 & 7.5 & 3 & 15.8 & 6.9 & 3 & 35.7 & 10.2 &  & 2.8 & 10.3 & 1-3,5 & 12.5 & 9.5 & 3 & \cellcolor{gray!20}{\textbf{0.6}} & 12.0 & 1-5\\

 &  &  & 5 & 10.2 & 7.8 & 2-3,5 & 13.1 & 7.1 & 3 & 38.0 & 12.9 &  & 3.4 & 10.9 & 2-3,5 & 13.8 & 10.1 & 3 & \cellcolor{gray!20}{\textbf{2.6}} & 11.2 & 2-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 14.3 & 8.1 & 3 & 10.9 & 6.8 & 3,5 & 39.3 & 15.3 &  & \cellcolor{gray!20}{\textbf{4.4}} & 10.6 & 1-3,5-6 & 13.4 & 9.4 & 3 & 5.5 & 10.0 & 1-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 12.7 & 5.2 & 2-3 & 22.4 & 5.3 & 3 & 31.0 & 6.2 &  & 1.5 & 10.6 & 1-3,5 & 15.1 & 9.5 & 2-3 & \cellcolor{gray!20}{\textbf{0.1}} & 11.2 & 1-5\\

 &  &  & 5 & 10.7 & 5.5 & 2-3,5 & 17.2 & 5.8 & 3 & 27.6 & 7.3 &  & 1.0 & 10.6 & 1-3,5 & 14.9 & 10.1 & 3 & \cellcolor{gray!20}{\textbf{0.8}} & 10.8 & 1-3,5\\

\multirow{-14}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{eil101-uncorr}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$75\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 8.8 & 5.2 & 2-3,5 & 17.1 & 6.4 & 3 & 26.4 & 7.6 &  & 0.9 & 10.8 & 1-3,5 & 13.6 & 10.1 & 2-3 & 0.9 & 11.0 & 1-3,5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{17.2}} & 7.1 & 2-6 & 22.4 & 6.8 & 3-6 & 35.4 & 8.7 & 5 & 36.1 & 29.0 & 5 & 43.6 & 18.6 &  & 31.8 & 18.6 & 3-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{15.6}} & 6.9 & 2-6 & 20.4 & 7.2 & 3-6 & 37.1 & 11.3 & 5 & 38.3 & 30.1 & 5 & 46.8 & 19.4 &  & 34.8 & 19.1 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{16.1}} & 7.8 & 3-6 & 17.9 & 7.8 & 3-6 & 43.2 & 12.9 &  & 39.8 & 30.6 & 3,5 & 49.8 & 19.9 &  & 36.5 & 19.3 & 3-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{12.2}} & 5.2 & 2-6 & 22.5 & 6.1 & 3-6 & 26.7 & 6.7 & 5 & 32.2 & 29.5 & 5 & 43.4 & 21.0 &  & 29.6 & 19.2 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{12.4}} & 5.5 & 2-6 & 21.9 & 6.1 & 3-6 & 26.6 & 7.3 & 4-5 & 33.2 & 29.4 & 5 & 44.4 & 21.3 &  & 31.8 & 20.0 & 5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$10\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{8.1}} & 5.0 & 2-6 & 20.0 & 6.1 & 3-6 & 27.4 & 7.2 & 4-5 & 33.2 & 29.1 & 5 & 43.5 & 21.2 &  & 29.5 & 19.3 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & 12.8 & 6.9 & 2-3 & 19.7 & 6.4 & 3 & 34.5 & 7.6 &  & 2.3 & 10.4 & 1-3,5 & 14.0 & 9.1 & 2-3 & \cellcolor{gray!20}{\textbf{0.4}} & 11.1 & 1-5\\

 &  &  & 5 & 13.7 & 7.2 & 2-3 & 17.8 & 7.3 & 3 & 31.4 & 10.2 &  & 2.5 & 10.6 & 1-3,5 & 14.8 & 9.7 & 2-3 & \cellcolor{gray!20}{\textbf{2.1}} & 10.7 & 1-3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 14.1 & 7.6 & 3 & 12.9 & 7.1 & 3,5 & 35.8 & 13.2 &  & \cellcolor{gray!20}{\textbf{3.1}} & 11.4 & 1-3,5 & 14.2 & 10.2 & 3 & 3.9 & 10.9 & 1-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 13.3 & 5.4 & 2-3,5 & 22.9 & 5.4 &  & 26.3 & 6.8 &  & 1.2 & 10.4 & 1-3,5 & 16.4 & 9.1 & 2-3 & \cellcolor{gray!20}{\textbf{1.0}} & 10.5 & 1-3,5\\

 &  &  & 5 & 13.5 & 4.9 & 2-3 & 19.6 & 5.5 & 3 & 26.8 & 7.1 &  & 1.4 & 10.5 & 1-3,5 & 15.6 & 9.8 & 2-3 & \cellcolor{gray!20}{\textbf{0.8}} & 11.1 & 1-3,5\\

\multirow{-14}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{eil101-usw}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$75\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 11.6 & 5.1 & 2-3 & 18.6 & 5.7 & 3 & 23.8 & 7.4 &  & \cellcolor{gray!20}{\textbf{0.8}} & 10.1 & 1-3,5 & 15.0 & 9.7 & 2-3 & 1.3 & 9.8 & 1-3,5\\
\midrule
 &  &  & 2 & \cellcolor{gray!20}{\textbf{18.3}} & 9.4 & 2-6 & 51.7 & 12.3 & 3,5 & 86.8 & 15.9 &  & 52.9 & 54.9 & 3,5 & 84.0 & 31.0 & 3 & 49.8 & 37.8 & 3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{18.7}} & 9.8 & 2-6 & 44.8 & 13.1 & 3-6 & 95.2 & 20.5 &  & 55.1 & 53.7 & 3,5 & 87.4 & 30.5 & 3 & 52.4 & 38.0 & 3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{17.9}} & 10.1 & 2-6 & 41.3 & 14.3 & 3-6 & 96.1 & 26.6 &  & 56.1 & 55.2 & 3,5 & 91.1 & 30.7 & 3 & 52.0 & 37.5 & 3-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{17.1}} & 8.5 & 2-6 & 68.2 & 12.3 & 3,5 & 78.6 & 14.6 & 5 & 49.1 & 55.8 & 2-3,5 & 95.5 & 35.1 &  & 49.0 & 38.1 & 2-3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{14.7}} & 6.9 & 2-6 & 61.4 & 13.2 & 3,5 & 65.9 & 15.2 & 5 & 48.9 & 56.3 & 2-3,5 & 97.4 & 35.1 &  & 52.1 & 38.4 & 2-3,5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{100\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{16.4}} & 8.1 & 2-6 & 55.5 & 14.2 & 3,5 & 69.1 & 18.8 & 5 & 49.5 & 55.5 & 2-3,5 & 95.6 & 34.4 &  & 44.6 & 36.0 & 2-5\\

\cmidrule{2-22}
 &  &  & 2 & 19.7 & 9.7 & 2-3,5 & 46.6 & 10.5 & 3 & 83.1 & 18.3 &  & 2.4 & 13.7 & 1-3,5 & 41.2 & 14.4 & 2-3 & \cellcolor{gray!20}{\textbf{-3.5}} & 17.1 & 1-5\\

 &  &  & 5 & 9.1 & 8.1 & 2-3,5 & 38.5 & 11.9 & 3 & 85.5 & 23.7 &  & 2.4 & 13.9 & 2-3,5 & 38.6 & 15.6 & 3 & \cellcolor{gray!20}{\textbf{0.7}} & 18.8 & 1-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 11.2 & 8.1 & 2-3,5 & 34.7 & 12.8 & 3,5 & 73.0 & 29.2 &  & \cellcolor{gray!20}{\textbf{1.5}} & 14.6 & 2-3,5 & 38.3 & 16.4 & 3 & 2.6 & 17.0 & 2-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 16.5 & 6.8 & 2-3,5 & 61.5 & 9.5 & 3 & 65.7 & 12.7 &  & 2.2 & 13.9 & 1-3,5 & 54.5 & 14.9 & 2-3 & \cellcolor{gray!20}{\textbf{-3.6}} & 15.9 & 1-5\\

 &  &  & 5 & 11.7 & 6.3 & 2-3,5 & 59.2 & 10.3 &  & 58.7 & 13.5 &  & 0.9 & 14.0 & 1-3,5 & 53.0 & 15.7 & 2 & \cellcolor{gray!20}{\textbf{-2.4}} & 17.6 & 1-5\\

\multirow{-14}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{a280-bsc}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{750\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 17.4 & 6.3 & 2-3,5 & 49.8 & 12.1 & 3 & 64.4 & 16.1 &  & 0.0 & 14.3 & 1-3,5 & 48.5 & 16.6 & 3 & \cellcolor{gray!20}{\textbf{-1.9}} & 17.4 & 1-5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{20.0}} & 10.1 & 2-6 & 57.8 & 13.2 & 3,5 & 103.2 & 15.8 &  & 52.5 & 54.2 & 2-3,5 & 92.0 & 32.3 & 3 & 50.8 & 38.9 & 2-3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{14.2}} & 10.1 & 2-6 & 49.3 & 14.7 & 3-5 & 96.4 & 20.9 &  & 53.6 & 53.5 & 3,5 & 95.3 & 31.2 &  & 51.6 & 38.4 & 3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{11.5}} & 9.6 & 2-6 & 48.4 & 15.7 & 3-5 & 94.4 & 28.0 &  & 54.3 & 56.3 & 3,5 & 99.1 & 33.9 &  & 51.0 & 37.1 & 3,5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{14.4}} & 7.3 & 2-6 & 73.5 & 11.9 & 5 & 69.9 & 14.7 & 5 & 49.1 & 55.6 & 2-3,5 & 105.1 & 35.8 &  & 47.8 & 37.2 & 2-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{11.2}} & 7.3 & 2-6 & 64.2 & 14.2 & 5 & 66.7 & 13.3 & 5 & 48.9 & 55.9 & 2-3,5 & 104.2 & 36.3 &  & 48.3 & 38.3 & 2-3,5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{100\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{10.4}} & 8.2 & 2-6 & 63.1 & 15.3 & 5 & 54.0 & 18.6 & 5 & 49.2 & 56.5 & 2,5 & 104.7 & 36.8 &  & 48.2 & 35.6 & 2,5\\

\cmidrule{2-22}
 &  &  & 2 & 12.7 & 7.6 & 2-3,5 & 53.0 & 11.0 & 3 & 85.5 & 17.0 &  & 2.4 & 13.6 & 1-3,5 & 47.5 & 14.6 & 2-3 & \cellcolor{gray!20}{\textbf{-0.9}} & 17.8 & 1-5\\

 &  &  & 5 & 11.6 & 7.9 & 2-3,5 & 43.1 & 12.7 & 3 & 88.1 & 19.9 &  & 1.5 & 13.8 & 1-3,5 & 44.9 & 16.0 & 3 & \cellcolor{gray!20}{\textbf{0.4}} & 15.9 & 1-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 7.4 & 9.9 & 2-3,5 & 38.1 & 14.3 & 3,5 & 86.9 & 24.4 &  & \cellcolor{gray!20}{\textbf{0.8}} & 14.8 & 1-3,5-6 & 43.7 & 18.1 & 3 & 3.4 & 17.3 & 2-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 13.9 & 6.2 & 2-3,5 & 68.9 & 10.4 &  & 57.2 & 12.2 &  & 1.8 & 13.2 & 1-3,5 & 60.4 & 15.6 & 2 & \cellcolor{gray!20}{\textbf{-0.2}} & 18.2 & 1-5\\

 &  &  & 5 & 13.0 & 6.1 & 2-3,5 & 64.1 & 11.9 &  & 52.2 & 14.0 & 2 & -0.1 & 14.5 & 1-3,5 & 57.9 & 17.2 & 2 & \cellcolor{gray!20}{\textbf{-0.9}} & 17.4 & 1-3,5\\

\multirow{-14}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{a280-uncorr}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{750\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 15.6 & 6.4 & 2-3,5 & 54.0 & 12.8 &  & 53.4 & 14.1 &  & \cellcolor{gray!20}{\textbf{0.2}} & 14.4 & 1-3,5 & 55.5 & 17.6 &  & 0.6 & 18.2 & 1-3,5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{12.1}} & 8.2 & 2-6 & 66.4 & 13.4 & 3,5 & 91.6 & 14.1 &  & 51.7 & 55.5 & 2-3,5 & 99.1 & 34.2 &  & 49.4 & 36.7 & 2-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{19.0}} & 9.2 & 2-6 & 57.2 & 14.8 & 3,5 & 95.4 & 20.0 &  & 53.3 & 55.8 & 3,5 & 100.4 & 33.9 &  & 50.3 & 36.4 & 2-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{7.9}} & 10.2 & 2-6 & 52.1 & 16.2 & 3,5 & 78.5 & 25.0 & 5 & 52.7 & 56.6 & 3,5 & 104.6 & 35.1 &  & 52.1 & 39.4 & 3,5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{14.6}} & 7.9 & 2-6 & 71.8 & 12.2 & 5 & 63.0 & 12.0 & 2,5 & 50.9 & 56.3 & 2-3,5 & 110.4 & 37.5 &  & 49.6 & 36.2 & 2-3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{15.2}} & 7.6 & 2-6 & 65.8 & 14.1 & 5 & 55.7 & 13.9 & 5 & 50.1 & 57.6 & 2,5 & 111.5 & 38.6 &  & 52.0 & 35.5 & 2,5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{100\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{14.1}} & 7.9 & 2-6 & 64.1 & 15.7 & 5 & 63.3 & 15.3 & 5 & 50.3 & 57.4 & 2-3,5 & 111.3 & 38.2 &  & 51.3 & 36.3 & 2-3,5\\

\cmidrule{2-22}
 &  &  & 2 & 16.3 & 6.2 & 2-3,5 & 56.0 & 11.5 & 3 & 86.8 & 14.0 &  & 2.2 & 14.0 & 1-3,5 & 53.3 & 15.7 & 3 & \cellcolor{gray!20}{\textbf{-0.2}} & 19.5 & 1-5\\

 &  &  & 5 & 9.1 & 7.2 & 2-3,5 & 45.5 & 12.4 & 3,5 & 79.7 & 23.1 &  & 1.4 & 15.0 & 1-3,5 & 49.0 & 17.3 & 3 & \cellcolor{gray!20}{\textbf{0.7}} & 17.2 & 1-3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 7.8 & 9.0 & 2-3,5 & 44.4 & 13.3 & 3,5 & 76.7 & 23.2 &  & \cellcolor{gray!20}{\textbf{0.2}} & 15.3 & 2-3,5-6 & 48.9 & 18.4 & 3 & 3.2 & 17.9 & 2-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 15.0 & 5.1 & 2-3,5 & 67.9 & 9.8 &  & 64.4 & 10.3 &  & 2.3 & 14.0 & 1-3,5 & 62.9 & 16.9 & 2 & \cellcolor{gray!20}{\textbf{1.2}} & 17.5 & 1-5\\

 &  &  & 5 & 16.9 & 5.4 & 2-3,5 & 63.7 & 11.2 &  & 49.0 & 11.3 & 2,5 & 1.8 & 14.6 & 1-3,5 & 61.5 & 18.2 &  & \cellcolor{gray!20}{\textbf{1.3}} & 17.6 & 1-3,5\\

\multirow{-14}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{a280-usw}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{750\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 12.2 & 5.4 & 2-3,5 & 59.1 & 12.0 &  & 43.3 & 10.1 & 2,5 & \cellcolor{gray!20}{\textbf{0.7}} & 15.5 & 1-3,5 & 58.0 & 19.1 &  & 1.1 & 17.5 & 1-3,5\\
\bottomrule
\end{tabular}
\end{scriptsize}
%\end{tiny}
\end{table*}

==> tables/perf_a280_m1395.tex <==
\begin{table*}[htbp]
\renewcommand{\arraystretch}{1.15}
\renewcommand{\tabcolsep}{5.6pt}
\caption{\label{tab:a280}Mean (\textbf{mean}), standard deviation (\textbf{std}) and results of Wilcoxon-Mann-Whitney tests at a significance level of $\alpha = 0.05$ (\textbf{stat}) in terms of relative performance for instance a280. Best, i.e. lowest, mean values are highlighted in \colorbox{gray!20}{\textbf{bold face}}. The entries in the stat-column are read as follows: a value of $S \in \{1, \ldots, 6\}$ means that algorithm $S$ performs significantly worse. Interval notation $S-T$ means that all algorithms in the interval perform worse.
}
\centering
\begin{scriptsize}
\begin{tabular}[t]{crrrrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{9}{c}{\textbf{(1+1) EA}} & \multicolumn{9}{c}{\textbf{(20+1)-EA}} \\
\cmidrule(l{3pt}r{3pt}){5-13} \cmidrule(l{3pt}r{3pt}){14-22}
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{3}{c}{\textbf{Inversion (1)}} & \multicolumn{3}{c}{\textbf{Exchange (2)}} & \multicolumn{3}{c}{\textbf{Jump (3)}} & \multicolumn{3}{c}{\textbf{Inversion (4)}} & \multicolumn{3}{c}{\textbf{Exchange (5)}} & \multicolumn{3}{c}{\textbf{Jump (6)}} \\
\cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10} \cmidrule(l{3pt}r{3pt}){11-13} \cmidrule(l{3pt}r{3pt}){14-16} \cmidrule(l{3pt}r{3pt}){17-19} \cmidrule(l{3pt}r{3pt}){20-22}
& $\tau$ & $[L, U]$ & $c$ & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat}\\
\midrule
 &  &  & 2 & \cellcolor{gray!20}{\textbf{49.8}} & 29.0 & 2-6 & 79.6 & 19.5 & 3-6 & 127.0 & 19.3 & 4-6 & 252.7 & 106.0 &  & 207.5 & 59.0 & 4 & 178.4 & 69.0 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{48.8}} & 32.2 & 2-6 & 81.6 & 20.8 & 3-6 & 142.7 & 25.3 & 4-6 & 262.4 & 103.9 &  & 221.0 & 57.9 & 4 & 187.5 & 68.9 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{44.0}} & 30.7 & 2-6 & 84.8 & 22.0 & 3-6 & 159.6 & 27.9 & 4-6 & 267.3 & 104.2 &  & 232.5 & 59.3 & 4 & 189.3 & 69.8 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{37.3}} & 28.3 & 2-6 & 93.0 & 21.9 & 3-6 & 99.8 & 26.8 & 4-6 & 242.1 & 108.0 &  & 216.3 & 66.7 & 4 & 165.8 & 75.5 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{43.2}} & 31.1 & 2-6 & 95.3 & 22.2 & 3-6 & 119.5 & 27.2 & 4-6 & 243.9 & 107.0 &  & 221.3 & 66.6 & 4 & 170.3 & 76.6 & 4-5\\

 & \multirow{-7}{*}{\raggedleft\arraybackslash \rotatebox{90}{10\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{41.8}} & 28.8 & 2-6 & 89.3 & 22.4 & 3-6 & 109.8 & 27.1 & 4-6 & 244.5 & 107.1 &  & 220.4 & 65.6 & 4 & 173.2 & 73.8 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{18.3}} & 9.4 & 2-6 & 51.7 & 12.3 & 3,5 & 86.8 & 15.9 &  & 52.9 & 54.9 & 3,5 & 84.0 & 31.0 & 3 & 49.8 & 37.8 & 3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{18.7}} & 9.8 & 2-6 & 44.8 & 13.1 & 3-6 & 95.2 & 20.5 &  & 55.1 & 53.7 & 3,5 & 87.4 & 30.5 & 3 & 52.4 & 38.0 & 3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{17.9}} & 10.1 & 2-6 & 41.3 & 14.3 & 3-6 & 96.1 & 26.6 &  & 56.1 & 55.2 & 3,5 & 91.1 & 30.7 & 3 & 52.0 & 37.5 & 3-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{17.1}} & 8.5 & 2-6 & 68.2 & 12.3 & 3,5 & 78.6 & 14.6 & 5 & 49.1 & 55.8 & 2-3,5 & 95.5 & 35.1 &  & 49.0 & 38.1 & 2-3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{14.7}} & 6.9 & 2-6 & 61.4 & 13.2 & 3,5 & 65.9 & 15.2 & 5 & 48.9 & 56.3 & 2-3,5 & 97.4 & 35.1 &  & 52.1 & 38.4 & 2-3,5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{100\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{16.4}} & 8.1 & 2-6 & 55.5 & 14.2 & 3,5 & 69.1 & 18.8 & 5 & 49.5 & 55.5 & 2-3,5 & 95.6 & 34.4 &  & 44.6 & 36.0 & 2-5\\

\cmidrule{2-22}
 &  &  & 2 & 19.7 & 9.7 & 2-3,5 & 46.6 & 10.5 & 3 & 83.1 & 18.3 &  & 2.4 & 13.7 & 1-3,5 & 41.2 & 14.4 & 2-3 & \cellcolor{gray!20}{\textbf{-3.5}} & 17.1 & 1-5\\

 &  &  & 5 & 9.1 & 8.1 & 2-3,5 & 38.5 & 11.9 & 3 & 85.5 & 23.7 &  & 2.4 & 13.9 & 2-3,5 & 38.6 & 15.6 & 3 & \cellcolor{gray!20}{\textbf{0.7}} & 18.8 & 1-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 11.2 & 8.1 & 2-3,5 & 34.7 & 12.8 & 3,5 & 73.0 & 29.2 &  & \cellcolor{gray!20}{\textbf{1.5}} & 14.6 & 2-3,5 & 38.3 & 16.4 & 3 & 2.6 & 17.0 & 2-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 16.5 & 6.8 & 2-3,5 & 61.5 & 9.5 & 3 & 65.7 & 12.7 &  & 2.2 & 13.9 & 1-3,5 & 54.5 & 14.9 & 2-3 & \cellcolor{gray!20}{\textbf{-3.6}} & 15.9 & 1-5\\

 &  &  & 5 & 11.7 & 6.3 & 2-3,5 & 59.2 & 10.3 &  & 58.7 & 13.5 &  & 0.9 & 14.0 & 1-3,5 & 53.0 & 15.7 & 2 & \cellcolor{gray!20}{\textbf{-2.4}} & 17.6 & 1-5\\

\multirow{-20}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{a280-bsc}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{750\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 17.4 & 6.3 & 2-3,5 & 49.8 & 12.1 & 3 & 64.4 & 16.1 &  & 0.0 & 14.3 & 1-3,5 & 48.5 & 16.6 & 3 & \cellcolor{gray!20}{\textbf{-1.9}} & 17.4 & 1-5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{43.1}} & 30.0 & 2-6 & 87.7 & 19.9 & 3-6 & 127.5 & 21.1 & 4-6 & 252.6 & 105.5 &  & 218.8 & 61.3 & 4 & 175.9 & 72.3 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{52.5}} & 31.6 & 2-6 & 88.0 & 21.7 & 3-6 & 140.1 & 25.9 & 4-6 & 259.1 & 103.9 &  & 229.4 & 58.6 & 4 & 181.2 & 70.9 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{40.4}} & 32.6 & 2-6 & 90.5 & 23.8 & 3-6 & 152.5 & 29.3 & 4-6 & 260.6 & 107.7 &  & 239.9 & 63.0 & 4 & 189.1 & 71.6 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{44.7}} & 29.7 & 2-6 & 100.2 & 22.3 & 3-6 & 105.9 & 25.8 & 4-6 & 244.5 & 108.6 &  & 226.8 & 66.5 & 4 & 167.6 & 78.3 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{35.4}} & 28.6 & 2-6 & 99.4 & 23.6 & 4-6 & 97.5 & 26.9 & 4-6 & 243.7 & 107.8 &  & 231.0 & 67.2 & 4 & 175.6 & 75.7 & 4-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{10\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{38.2}} & 28.1 & 2-6 & 100.0 & 24.2 & 4-6 & 99.8 & 28.8 & 4-6 & 243.9 & 107.7 &  & 234.6 & 67.0 & 4 & 174.0 & 77.1 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{20.0}} & 10.1 & 2-6 & 57.8 & 13.2 & 3,5 & 103.2 & 15.8 &  & 52.5 & 54.2 & 2-3,5 & 92.0 & 32.3 & 3 & 50.8 & 38.9 & 2-3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{14.2}} & 10.1 & 2-6 & 49.3 & 14.7 & 3-5 & 96.4 & 20.9 &  & 53.6 & 53.5 & 3,5 & 95.3 & 31.2 &  & 51.6 & 38.4 & 3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{11.5}} & 9.6 & 2-6 & 48.4 & 15.7 & 3-5 & 94.4 & 28.0 &  & 54.3 & 56.3 & 3,5 & 99.1 & 33.9 &  & 51.0 & 37.1 & 3,5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{14.4}} & 7.3 & 2-6 & 73.5 & 11.9 & 5 & 69.9 & 14.7 & 5 & 49.1 & 55.6 & 2-3,5 & 105.1 & 35.8 &  & 47.8 & 37.2 & 2-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{11.2}} & 7.3 & 2-6 & 64.2 & 14.2 & 5 & 66.7 & 13.3 & 5 & 48.9 & 55.9 & 2-3,5 & 104.2 & 36.3 &  & 48.3 & 38.3 & 2-3,5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{100\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{10.4}} & 8.2 & 2-6 & 63.1 & 15.3 & 5 & 54.0 & 18.6 & 5 & 49.2 & 56.5 & 2,5 & 104.7 & 36.8 &  & 48.2 & 35.6 & 2,5\\

\cmidrule{2-22}
 &  &  & 2 & 12.7 & 7.6 & 2-3,5 & 53.0 & 11.0 & 3 & 85.5 & 17.0 &  & 2.4 & 13.6 & 1-3,5 & 47.5 & 14.6 & 2-3 & \cellcolor{gray!20}{\textbf{-0.9}} & 17.8 & 1-5\\

 &  &  & 5 & 11.6 & 7.9 & 2-3,5 & 43.1 & 12.7 & 3 & 88.1 & 19.9 &  & 1.5 & 13.8 & 1-3,5 & 44.9 & 16.0 & 3 & \cellcolor{gray!20}{\textbf{0.4}} & 15.9 & 1-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 7.4 & 9.9 & 2-3,5 & 38.1 & 14.3 & 3,5 & 86.9 & 24.4 &  & \cellcolor{gray!20}{\textbf{0.8}} & 14.8 & 1-3,5-6 & 43.7 & 18.1 & 3 & 3.4 & 17.3 & 2-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 13.9 & 6.2 & 2-3,5 & 68.9 & 10.4 &  & 57.2 & 12.2 &  & 1.8 & 13.2 & 1-3,5 & 60.4 & 15.6 & 2 & \cellcolor{gray!20}{\textbf{-0.2}} & 18.2 & 1-5\\

 &  &  & 5 & 13.0 & 6.1 & 2-3,5 & 64.1 & 11.9 &  & 52.2 & 14.0 & 2 & -0.1 & 14.5 & 1-3,5 & 57.9 & 17.2 & 2 & \cellcolor{gray!20}{\textbf{-0.9}} & 17.4 & 1-3,5\\

\multirow{-20}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{a280-uncorr}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{750\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 15.6 & 6.4 & 2-3,5 & 54.0 & 12.8 &  & 53.4 & 14.1 &  & \cellcolor{gray!20}{\textbf{0.2}} & 14.4 & 1-3,5 & 55.5 & 17.6 &  & 0.6 & 18.2 & 1-3,5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{41.7}} & 29.8 & 2-6 & 93.0 & 21.9 & 3-6 & 120.4 & 22.1 & 4-6 & 248.7 & 106.6 &  & 225.2 & 63.8 & 4 & 173.3 & 74.3 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{42.7}} & 30.7 & 2-6 & 93.5 & 23.6 & 3-6 & 136.9 & 23.1 & 4-6 & 255.7 & 105.7 &  & 235.9 & 61.7 & 4 & 176.8 & 75.2 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{40.7}} & 32.1 & 2-6 & 95.0 & 25.1 & 3-6 & 140.2 & 29.3 & 4-6 & 257.5 & 106.7 &  & 242.6 & 64.1 & 4 & 188.6 & 71.8 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{40.9}} & 30.1 & 2-6 & 105.1 & 23.1 & 4-6 & 90.3 & 27.2 & 2,4-6 & 244.3 & 108.2 &  & 237.2 & 67.7 & 4 & 171.8 & 79.8 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{39.3}} & 29.9 & 2-6 & 102.7 & 25.6 & 4-6 & 88.7 & 26.7 & 2,4-6 & 247.6 & 110.0 &  & 239.1 & 68.4 & 4 & 177.5 & 77.3 & 4-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{10\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{40.3}} & 29.7 & 2-6 & 105.4 & 25.8 & 4-6 & 96.4 & 29.1 & 4-6 & 246.2 & 109.1 &  & 241.3 & 69.4 & 4 & 175.6 & 79.1 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{12.1}} & 8.2 & 2-6 & 66.4 & 13.4 & 3,5 & 91.6 & 14.1 &  & 51.7 & 55.5 & 2-3,5 & 99.1 & 34.2 &  & 49.4 & 36.7 & 2-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{19.0}} & 9.2 & 2-6 & 57.2 & 14.8 & 3,5 & 95.4 & 20.0 &  & 53.3 & 55.8 & 3,5 & 100.4 & 33.9 &  & 50.3 & 36.4 & 2-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{7.9}} & 10.2 & 2-6 & 52.1 & 16.2 & 3,5 & 78.5 & 25.0 & 5 & 52.7 & 56.6 & 3,5 & 104.6 & 35.1 &  & 52.1 & 39.4 & 3,5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{14.6}} & 7.9 & 2-6 & 71.8 & 12.2 & 5 & 63.0 & 12.0 & 2,5 & 50.9 & 56.3 & 2-3,5 & 110.4 & 37.5 &  & 49.6 & 36.2 & 2-3,5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{15.2}} & 7.6 & 2-6 & 65.8 & 14.1 & 5 & 55.7 & 13.9 & 5 & 50.1 & 57.6 & 2,5 & 111.5 & 38.6 &  & 52.0 & 35.5 & 2,5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{100\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{14.1}} & 7.9 & 2-6 & 64.1 & 15.7 & 5 & 63.3 & 15.3 & 5 & 50.3 & 57.4 & 2-3,5 & 111.3 & 38.2 &  & 51.3 & 36.3 & 2-3,5\\

\cmidrule{2-22}
 &  &  & 2 & 16.3 & 6.2 & 2-3,5 & 56.0 & 11.5 & 3 & 86.8 & 14.0 &  & 2.2 & 14.0 & 1-3,5 & 53.3 & 15.7 & 3 & \cellcolor{gray!20}{\textbf{-0.2}} & 19.5 & 1-5\\

 &  &  & 5 & 9.1 & 7.2 & 2-3,5 & 45.5 & 12.4 & 3,5 & 79.7 & 23.1 &  & 1.4 & 15.0 & 1-3,5 & 49.0 & 17.3 & 3 & \cellcolor{gray!20}{\textbf{0.7}} & 17.2 & 1-3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 7.8 & 9.0 & 2-3,5 & 44.4 & 13.3 & 3,5 & 76.7 & 23.2 &  & \cellcolor{gray!20}{\textbf{0.2}} & 15.3 & 2-3,5-6 & 48.9 & 18.4 & 3 & 3.2 & 17.9 & 2-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 15.0 & 5.1 & 2-3,5 & 67.9 & 9.8 &  & 64.4 & 10.3 &  & 2.3 & 14.0 & 1-3,5 & 62.9 & 16.9 & 2 & \cellcolor{gray!20}{\textbf{1.2}} & 17.5 & 1-5\\

 &  &  & 5 & 16.9 & 5.4 & 2-3,5 & 63.7 & 11.2 &  & 49.0 & 11.3 & 2,5 & 1.8 & 14.6 & 1-3,5 & 61.5 & 18.2 &  & \cellcolor{gray!20}{\textbf{1.3}} & 17.6 & 1-3,5\\

\multirow{-22}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{a280-usw}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{750\,000}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 12.2 & 5.4 & 2-3,5 & 59.1 & 12.0 &  & 43.3 & 10.1 & 2,5 & \cellcolor{gray!20}{\textbf{0.7}} & 15.5 & 1-3,5 & 58.0 & 19.1 &  & 1.1 & 17.5 & 1-3,5\\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{table*}

==> tables/perf_eil101_m500.tex <==
\begin{table*}[htbp]
\renewcommand{\arraystretch}{1.15}
\renewcommand{\tabcolsep}{5.6pt}
\caption{\label{tab:eil101}Mean (\textbf{mean}), standard deviation (\textbf{std}) and results of Wilcoxon-Mann-Whitney tests at a significance level of $\alpha = 0.05$ (\textbf{stat}) in terms of relative performance for instance eil101. Best, i.e. lowest, mean values are highlighted in \colorbox{gray!20}{\textbf{bold face}}. The entries in the stat-column are read as follows: a value of $S \in \{1, \ldots, 6\}$ means that algorithm $S$ performs significantly worse. Interval notation $S-T$ means that all algorithms in the interval perform worse.}
\centering
%\begin{scriptsize}
\begin{scriptsize}
\begin{tabular}[t]{crrrrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{9}{c}{\textbf{(1+1) EA}} & \multicolumn{9}{c}{\textbf{(20+1)-EA}} \\
\cmidrule(l{3pt}r{3pt}){5-13} \cmidrule(l{3pt}r{3pt}){14-22}
\multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{1}{c}{\textbf{ }} & \multicolumn{3}{c}{\textbf{Inversion (1)}} & \multicolumn{3}{c}{\textbf{Exchange (2)}} & \multicolumn{3}{c}{\textbf{Jump (3)}} & \multicolumn{3}{c}{\textbf{Inversion (4)}} & \multicolumn{3}{c}{\textbf{Exchange (5)}} & \multicolumn{3}{c}{\textbf{Jump (6)}} \\
\cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10} \cmidrule(l{3pt}r{3pt}){11-13} \cmidrule(l{3pt}r{3pt}){14-16} \cmidrule(l{3pt}r{3pt}){17-19} \cmidrule(l{3pt}r{3pt}){20-22}
& $\tau$ & $[L, U]$ & $c$ & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat} & \textbf{mean} & \textbf{std} & \textbf{stat}\\
\midrule
 &  &  & 2 & 36.2 & 9.7 & 3-6 & \cellcolor{gray!20}{\textbf{31.7}} & 8.5 & 1,3-6 & 54.9 & 11.8 & 4-6 & 134.1 & 27.6 &  & 106.8 & 17.6 & 4 & 98.8 & 19.9 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{32.8}} & 10.5 & 2-6 & 38.5 & 9.4 & 3-6 & 64.5 & 15.6 & 4-6 & 140.9 & 27.5 &  & 116.1 & 18.5 & 4 & 102.6 & 22.5 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{33.8}} & 11.7 & 2-6 & 42.1 & 10.4 & 3-6 & 76.9 & 18.1 & 4-6 & 147.5 & 29.0 &  & 124.2 & 20.8 & 4 & 109.1 & 21.6 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{23.4}} & 8.1 & 2-6 & 32.3 & 6.9 & 3-6 & 46.7 & 7.7 & 4-6 & 119.7 & 26.9 &  & 101.5 & 19.1 & 4 & 88.6 & 21.0 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{24.0}} & 7.8 & 2-6 & 31.3 & 7.7 & 3-6 & 40.2 & 8.3 & 4-6 & 122.4 & 28.3 &  & 103.5 & 19.6 & 4 & 87.5 & 20.6 & 4-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$1\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{24.6}} & 8.0 & 2-6 & 34.2 & 8.5 & 3-6 & 42.3 & 7.9 & 4-6 & 123.2 & 28.6 &  & 105.1 & 20.7 & 4 & 89.3 & 21.9 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & 22.8 & 9.5 & 3-6 & \cellcolor{gray!20}{\textbf{16.0}} & 7.3 & 1,3-6 & 38.0 & 11.2 &  & 39.7 & 30.0 &  & 40.0 & 19.2 &  & 35.7 & 17.7 & 4-5\\

 &  &  & 5 & 18.8 & 9.0 & 3-6 & \cellcolor{gray!20}{\textbf{15.6}} & 7.6 & 3-6 & 43.8 & 14.3 &  & 41.6 & 29.6 & 5 & 44.9 & 18.7 &  & 38.6 & 18.3 & 3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 16.7 & 10.0 & 3-6 & \cellcolor{gray!20}{\textbf{15.3}} & 8.1 & 3-6 & 49.2 & 16.7 &  & 45.8 & 30.5 & 3,5 & 50.2 & 19.2 &  & 42.6 & 19.0 & 3-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{19.1}} & 6.7 & 3-6 & 21.8 & 6.1 & 3-6 & 35.3 & 7.8 &  & 34.3 & 30.4 & 5 & 40.2 & 20.0 &  & 30.0 & 19.4 & 3-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{13.3}} & 5.6 & 2-6 & 19.2 & 6.6 & 3-6 & 31.5 & 8.4 & 5 & 34.1 & 29.7 & 5 & 41.1 & 20.4 &  & 29.1 & 19.4 & 3-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$10\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{11.5}} & 6.1 & 2-6 & 19.2 & 7.3 & 3-6 & 29.5 & 10.1 & 5 & 33.7 & 30.1 & 5 & 42.0 & 21.1 &  & 32.7 & 19.5 & 5\\

\cmidrule{2-22}
 &  &  & 2 & 20.8 & 8.1 & 3 & 15.6 & 7.1 & 3 & 38.2 & 11.4 &  & 3.0 & 10.8 & 1-3,5 & 11.0 & 9.3 & 2-3 & \cellcolor{gray!20}{\textbf{-0.3}} & 12.4 & 1-5\\

 &  &  & 5 & 15.9 & 8.7 & 3 & 14.0 & 7.5 & 3 & 38.8 & 13.1 &  & 3.6 & 11.1 & 1-3,5 & 12.3 & 9.6 & 3 & \cellcolor{gray!20}{\textbf{1.5}} & 10.7 & 1-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 15.4 & 9.9 & 3 & 9.3 & 7.3 & 3,5 & 42.7 & 16.4 &  & \cellcolor{gray!20}{\textbf{4.6}} & 11.3 & 1-3,5 & 12.7 & 9.9 & 3 & 5.5 & 10.2 & 1-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 14.2 & 5.8 & 2-3 & 21.1 & 5.9 & 3 & 33.4 & 7.3 &  & 1.7 & 10.6 & 1-3,5 & 13.9 & 9.4 & 2-3 & \cellcolor{gray!20}{\textbf{-0.9}} & 11.9 & 1-5\\

 &  &  & 5 & 13.8 & 6.3 & 3 & 14.4 & 6.4 & 3 & 29.3 & 7.7 &  & 0.6 & 10.4 & 1-3,5 & 12.9 & 9.4 & 3 & \cellcolor{gray!20}{\textbf{-0.6}} & 11.4 & 1-5\\

\multirow{-21}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{eil101-bsc}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$75\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 13.2 & 6.0 & 3 & 16.2 & 6.2 & 3 & 28.4 & 8.5 &  & 0.8 & 10.9 & 1-3,5 & 12.4 & 9.9 & 2-3 & \cellcolor{gray!20}{\textbf{0.2}} & 11.6 & 1-3,5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{26.7}} & 8.1 & 2-6 & 32.3 & 7.4 & 3-6 & 53.9 & 9.4 & 4-6 & 129.7 & 26.8 &  & 106.0 & 17.3 & 4 & 95.4 & 20.2 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{31.5}} & 9.9 & 2-6 & 38.4 & 8.8 & 3-6 & 62.6 & 14.4 & 4-6 & 135.2 & 29.6 &  & 114.5 & 19.1 & 4 & 100.4 & 21.4 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{34.7}} & 11.2 & 2-6 & 40.3 & 9.6 & 3-6 & 78.0 & 18.7 & 4-6 & 139.2 & 26.7 &  & 122.8 & 18.5 & 4 & 105.8 & 20.9 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{22.3}} & 7.4 & 2-6 & 34.1 & 7.2 & 3-6 & 42.2 & 7.6 & 4-6 & 116.1 & 27.0 &  & 103.6 & 18.6 & 4 & 87.7 & 20.4 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{19.9}} & 7.4 & 2-6 & 34.1 & 7.3 & 3-6 & 39.9 & 8.3 & 4-6 & 118.1 & 28.3 &  & 103.7 & 18.8 & 4 & 86.2 & 21.6 & 4-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$1\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{20.8}} & 7.3 & 2-6 & 35.8 & 7.6 & 3-6 & 39.9 & 7.9 & 4-6 & 121.2 & 28.6 &  & 102.9 & 20.0 & 4 & 89.5 & 21.1 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{15.4}} & 7.0 & 2-6 & 21.5 & 7.0 & 3-6 & 41.2 & 10.7 &  & 38.1 & 29.3 & 5 & 41.7 & 19.0 &  & 32.5 & 18.4 & 3-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{16.8}} & 8.7 & 3-6 & 17.9 & 8.1 & 3-6 & 42.8 & 12.1 &  & 39.6 & 29.4 & 3,5 & 46.3 & 19.4 &  & 36.7 & 18.2 & 3-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{15.1}} & 7.3 & 3-6 & 16.0 & 7.7 & 3-6 & 45.2 & 15.4 &  & 43.8 & 28.7 & 5 & 50.9 & 18.5 &  & 40.4 & 18.3 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{14.8}} & 4.9 & 3-6 & 19.6 & 5.6 & 3-6 & 32.6 & 6.7 & 5 & 32.3 & 29.6 & 5 & 42.6 & 20.9 &  & 29.9 & 18.9 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{11.7}} & 5.7 & 2-6 & 21.9 & 6.5 & 3-6 & 27.3 & 7.9 & 4-6 & 32.3 & 29.0 & 5 & 44.3 & 21.6 &  & 30.3 & 19.1 & 4-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$10\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{8.4}} & 6.8 & 2-6 & 18.7 & 7.3 & 3-6 & 29.7 & 8.4 & 5 & 33.4 & 29.9 & 5 & 43.9 & 21.4 &  & 31.4 & 18.7 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & 17.8 & 7.5 & 3 & 15.8 & 6.9 & 3 & 35.7 & 10.2 &  & 2.8 & 10.3 & 1-3,5 & 12.5 & 9.5 & 3 & \cellcolor{gray!20}{\textbf{0.6}} & 12.0 & 1-5\\

 &  &  & 5 & 10.2 & 7.8 & 2-3,5 & 13.1 & 7.1 & 3 & 38.0 & 12.9 &  & 3.4 & 10.9 & 2-3,5 & 13.8 & 10.1 & 3 & \cellcolor{gray!20}{\textbf{2.6}} & 11.2 & 2-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 14.3 & 8.1 & 3 & 10.9 & 6.8 & 3,5 & 39.3 & 15.3 &  & \cellcolor{gray!20}{\textbf{4.4}} & 10.6 & 1-3,5-6 & 13.4 & 9.4 & 3 & 5.5 & 10.0 & 1-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 12.7 & 5.2 & 2-3 & 22.4 & 5.3 & 3 & 31.0 & 6.2 &  & 1.5 & 10.6 & 1-3,5 & 15.1 & 9.5 & 2-3 & \cellcolor{gray!20}{\textbf{0.1}} & 11.2 & 1-5\\

 &  &  & 5 & 10.7 & 5.5 & 2-3,5 & 17.2 & 5.8 & 3 & 27.6 & 7.3 &  & 1.0 & 10.6 & 1-3,5 & 14.9 & 10.1 & 3 & \cellcolor{gray!20}{\textbf{0.8}} & 10.8 & 1-3,5\\

\multirow{-21}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{eil101-uncorr}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$75\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 8.8 & 5.2 & 2-3,5 & 17.1 & 6.4 & 3 & 26.4 & 7.6 &  & 0.9 & 10.8 & 1-3,5 & 13.6 & 10.1 & 2-3 & 0.9 & 11.0 & 1-3,5\\
\cmidrule{1-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{23.0}} & 7.6 & 2-6 & 35.2 & 7.5 & 3-6 & 49.0 & 9.3 & 4-6 & 123.6 & 25.9 &  & 107.8 & 17.5 & 4 & 92.9 & 19.6 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{27.5}} & 8.7 & 2-6 & 36.8 & 8.2 & 3-6 & 56.2 & 11.5 & 4-6 & 129.2 & 27.1 &  & 112.7 & 18.0 & 4 & 96.2 & 23.0 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{30.0}} & 9.8 & 2-6 & 40.7 & 10.5 & 3-6 & 67.2 & 13.6 & 4-6 & 133.2 & 28.9 &  & 118.1 & 20.7 & 4 & 100.3 & 22.7 & 4-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{18.1}} & 6.6 & 2-6 & 36.3 & 7.1 & 4-6 & 38.9 & 8.4 & 4-6 & 117.5 & 26.0 &  & 103.5 & 18.5 & 4 & 87.6 & 20.4 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{19.7}} & 7.5 & 2-6 & 34.3 & 7.4 & 4-6 & 36.0 & 7.6 & 4-6 & 119.0 & 27.6 &  & 105.8 & 19.3 & 4 & 87.7 & 20.9 & 4-5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$1\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{21.3}} & 6.9 & 2-6 & 34.8 & 7.7 & 4-6 & 37.7 & 7.4 & 4-6 & 119.0 & 26.7 &  & 105.1 & 18.8 & 4 & 89.5 & 20.9 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{17.2}} & 7.1 & 2-6 & 22.4 & 6.8 & 3-6 & 35.4 & 8.7 & 5 & 36.1 & 29.0 & 5 & 43.6 & 18.6 &  & 31.8 & 18.6 & 3-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{15.6}} & 6.9 & 2-6 & 20.4 & 7.2 & 3-6 & 37.1 & 11.3 & 5 & 38.3 & 30.1 & 5 & 46.8 & 19.4 &  & 34.8 & 19.1 & 4-5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & \cellcolor{gray!20}{\textbf{16.1}} & 7.8 & 3-6 & 17.9 & 7.8 & 3-6 & 43.2 & 12.9 &  & 39.8 & 30.6 & 3,5 & 49.8 & 19.9 &  & 36.5 & 19.3 & 3-5\\

\cmidrule{3-22}
 &  &  & 2 & \cellcolor{gray!20}{\textbf{12.2}} & 5.2 & 2-6 & 22.5 & 6.1 & 3-6 & 26.7 & 6.7 & 5 & 32.2 & 29.5 & 5 & 43.4 & 21.0 &  & 29.6 & 19.2 & 4-5\\

 &  &  & 5 & \cellcolor{gray!20}{\textbf{12.4}} & 5.5 & 2-6 & 21.9 & 6.1 & 3-6 & 26.6 & 7.3 & 4-5 & 33.2 & 29.4 & 5 & 44.4 & 21.3 &  & 31.8 & 20.0 & 5\\

 & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$10\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & \cellcolor{gray!20}{\textbf{8.1}} & 5.0 & 2-6 & 20.0 & 6.1 & 3-6 & 27.4 & 7.2 & 4-5 & 33.2 & 29.1 & 5 & 43.5 & 21.2 &  & 29.5 & 19.3 & 4-5\\

\cmidrule{2-22}
 &  &  & 2 & 12.8 & 6.9 & 2-3 & 19.7 & 6.4 & 3 & 34.5 & 7.6 &  & 2.3 & 10.4 & 1-3,5 & 14.0 & 9.1 & 2-3 & \cellcolor{gray!20}{\textbf{0.4}} & 11.1 & 1-5\\

 &  &  & 5 & 13.7 & 7.2 & 2-3 & 17.8 & 7.3 & 3 & 31.4 & 10.2 &  & 2.5 & 10.6 & 1-3,5 & 14.8 & 9.7 & 2-3 & \cellcolor{gray!20}{\textbf{2.1}} & 10.7 & 1-3,5\\

 &  & \multirow{-3}{*}{\raggedleft\arraybackslash $[30, 70]$} & 10 & 14.1 & 7.6 & 3 & 12.9 & 7.1 & 3,5 & 35.8 & 13.2 &  & \cellcolor{gray!20}{\textbf{3.1}} & 11.4 & 1-3,5 & 14.2 & 10.2 & 3 & 3.9 & 10.9 & 1-3,5\\

\cmidrule{3-22}
 &  &  & 2 & 13.3 & 5.4 & 2-3,5 & 22.9 & 5.4 &  & 26.3 & 6.8 &  & 1.2 & 10.4 & 1-3,5 & 16.4 & 9.1 & 2-3 & \cellcolor{gray!20}{\textbf{1.0}} & 10.5 & 1-3,5\\

 &  &  & 5 & 13.5 & 4.9 & 2-3 & 19.6 & 5.5 & 3 & 26.8 & 7.1 &  & 1.4 & 10.5 & 1-3,5 & 15.6 & 9.8 & 2-3 & \cellcolor{gray!20}{\textbf{0.8}} & 11.1 & 1-3,5\\

\multirow{-22}{*}{\centering\arraybackslash \rotatebox{90}{\textbf{eil101-usw}}} & \multirow{-6}{*}{\raggedleft\arraybackslash \rotatebox{90}{$75\,000$}} & \multirow{-3}{*}{\raggedleft\arraybackslash $[70, 90]$} & 10 & 11.6 & 5.1 & 2-3 & 18.6 & 5.7 & 3 & 23.8 & 7.4 &  & \cellcolor{gray!20}{\textbf{0.8}} & 10.1 & 1-3,5 & 15.0 & 9.7 & 2-3 & 1.3 & 9.8 & 1-3,5\\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{table*}
